Regulating Transportation Network Companies with a Mixture of Autonomous Vehicles and For-Hire Human Drivers

This paper investigates the equity impacts of autonomous vehicles (AV) on for-hire human drivers and passengers in a ride-hailing market, and examines regulation policies that protect human drivers and improve transport equity for ride-hailing passengers. We consider a transportation network companies (TNC) that employs a mixture of AVs and human drivers to provide ride-hailing services. The TNC platform determines the spatial prices, fleet size, human driver payments, and vehicle relocation strategies to maximize its profit, while individual passengers choose between different transport modes to minimize their travel costs. A market equilibrium model is proposed to capture the interactions among passengers, human drivers, AVs, and TNC over the transportation network. The overall problem is formulated as a non-concave program, and an algorithm is developed to derive its approximate solution with a theoretical performance guarantee. Our study shows that TNC prioritizes AV deployment in higher-demand areas to make a higher profit. As AVs flood into these higher-demand areas, they compete with human drivers in the urban core and push them to relocate to suburbs. This leads to reduced earning opportunities for human drivers and increased spatial inequity for passengers. To mitigate these concerns, we consider: (a) a minimum wage for human drivers; and (b) a restrictive pickup policy that prohibits AVs from picking up passengers in higher-demand areas. In the former case, we show that a minimum wage for human drivers will protect them from the negative impact of AVs with negligible impacts on passengers. However, there exists a threshold beyond which the minimum wage will trigger the platform to replace the majority of human drivers with AVs.

==> Introduction.tex <==
\section{Introduction}


In December 2018, New York   became the first city in the U.S. to adopt a minimum wage for drivers working for app-based transportation network companies (TNCs) like Uber and Lyft. The New York City Taxi and Limousine Commission (NYTLC) established a ``minimum per-trip payment formula'' that gave an estimated gross hourly driver earnings before expenses of at least \$26.51 per hour and a net income of 
\$17.22 per hour after expenses, equivalent to the minimum wage of \$15 per hour because, as ``independent contractors,'' drivers pay additional payroll taxes and get no paid time off. 
The NYTLC formula for non-wheelchair accessible vehicles is
\begin{equation}\label{utilization}
\mbox{Driver pay per trip} =
\Bigg( \frac{\$0.631 \times \text{Trip Miles}}{\text{Company Utilization Rate}}\Bigg)
+ \Bigg( \frac{\$0.287 \times \text{Trip Minutes}}{\text{Company Utilization Rate}}\Bigg)
+ \text{Shared Ride Bonus},
\end{equation}
amounting to \$23 for a 30-min, 7.5-mile ride.\footnote{The utilization rate is calculated by dividing the total amount of time drivers spend transporting passengers on trips dispatched by the base by the total amount of time drivers are available to accept dispatches from the base \cite{ban2018gan}.}


The Commission imposed the wage floor based on  testimony  on driver expenses, meetings with stakeholders, and on the report of  labor economists J.A. Parrott and M. Reich which showed that
median driver earnings had declined almost \$3.00 per hour from \$25.78 in September  2016 to \$ 22.90 in October 2017, a decrease of 11.17\%.   The TNCs imposed the \$3.00 per hour wage cut  
during a period when the number of  drivers in the largest four TNCs (Uber, Lyft, Gett/Juno, and Via) had grown by 80,000 \cite{ban2018gan}. Uber  would be the largest for-profit private employer in New York City if its drivers were classified as employees rather than independent contractors \cite{parrott2018earning}.

The subminimum wage of Uber drivers also prompted the Seattle City Council in April 2018  to pass a unanimous resolution to explore setting a minimum base rate  of \$2.40 per mile for TNCs compared with the prevailing rate of \$1.35 per mile and the rate of \$2.70 charged by taxis.  The resolution also asked TNCs to voluntarily hand over anonymous data on hours, trips, fares and compensation.  Unlike NYTLC, however, no other US city has access to TNC data to estimate what their drivers are paid.

In December 2018, Uber lost its case at the U.K.'s Court of Appeal  against the  October, 2016, ruling that its drivers should be classified as workers entitled to rights such as minimum wage and paid holidays.  The Court ruled against Uber's claim that its drivers were just self-employed contractors who use its app in exchange for a share of their fares at the level dictated by Uber \cite{Uber_London}. The case can be used to challenge the self-employed status of millions of gig-economy workers who  work for companies like Airbnb and Deliveroo on a freelance basis without fixed contracts.
New York and London are the largest Uber markets in the U.S. and E.U.

Uber's reaction to these three adverse decisions was predictable.
Responding to the NYTLC ruling Uber's director of public affairs stated, ``legislation to increase driver earnings will lead to higher than necessary fare increases for riders while missing an opportunity to deal with congestion in Manhattan's central business district.''\footnote{Lyft echoed the Uber response 
stating, ``These rules would be a step backward for New Yorkers, and we urge the TLC to reconsider them \cite{Uber_USA}.''}  Uber  challenged the Seattle resolution: its general manager for  Seattle said, ``we are generally unclear how nearly doubling per-mile rider rates would not result in an increased cost for riders.''  Uber also declared it would fight the U.K. Appeal Court's decision in the Supreme Court. Contradicting Uber's claims, this study shows that, for a large range of parameter values, raising driver wages will \textit{increase} the number of drivers at the same time that passengers enjoy \textit{faster} and \textit{cheaper} rides, while platform rents are reduced. 

The aforementioned regulations are partly motivated by public concern over the disruption to the urban transportation system caused by the rapid growth of RNCs. Worldwide, the
monthly number of Uber users  is forecast to reach 100 million in 2018, up from 75 million in 2017. In New York, Uber, Lyft,  Juno and Via combined dispatched nearly 600,000  rides per day in the first quarter of 2018, increasing their annual trip totals by over 100 percent in 2016 and by 71 percent in 2017. About 80,000 vehicles are affiliated with these four companies \cite{parrott2018earning}.  In San Francisco, 5,700 TNC vehicles operate in peak times.  They daily make over 170,000 vehicle trips, approximately 12 times the number of taxi trips, and 15 percent of all intra-San Francisco  trips, comprising  
at least 9 percent of all San Francisco person trips \cite{castiglione2016tncs}.  This explosive growth of TNCs has raised two  public concerns.  

As noted above, one concern is with the working conditions of TNC drivers.  The TNC  business model  places much of the economic risk associated with the app sector on  drivers, who are classified as independent contractors. Furthermore, the model relies on having many idle cars and drivers,  resulting in low driver pay per hour and high TNC platform rents.\footnote{TNC expenditures comprise a fixed initial cost for setting up the platform and a small variable cost as the company grows.  Thus the  average cost per trip falls and its profit margin increases as the TNC grows.} Uber's annual revenue from passenger fares in New York City amounts to about \$2
billion, of which it keeps about \$375 million in commissions and fees, for a markup  estimated at six times its variable operating cost or 600 percent \cite{parrott2018earning}. 
One common understanding is that ``Uber's driver-partners are attracted to the flexible schedules that driving on the Uber platform affords \ldots because the nature of the work, the flexibility, and the compensation appeals to them compared with other available options \cite{Hall_Kreuger}.''
  In fact, more than 60 percent of  New York City drivers  work full-time and provide 80 percent of all rides; their work hours are not flexible \cite{parrott2018earning}.


The second concern is with the negative impact of the explosive TNC growth on a city's traffic congestion as well as public transit ridership.
A detailed 2017 report  \cite{schaller2017empty}  examined the impact of TNC growth on traffic conditions in Manhattan's CBD. The analysis shows that, from 2013 to 2017, TNC trips increased  15 percent, VMT increased  36 percent, traffic speed declined 15 percent, the number of vehicles increased  59 percent, and the number of unoccupied vehicles increased  81 percent. The report suggested reducing the unoccupied time of TNC vehicles as a means of congestion control. Responding to the increased congestion, the New York City Council in 2018 passed  a regulation freezing the number of TNC vehicles on the road for one year. Supporters of the cap, including Mayor Bill de Blasio,  said the regulation will protect drivers, fairly regulate the industry and reduce congestion \cite{cnbc_NY}.  However, our analysis shows that imposing a cap hurts drivers, because the TNC retains as profit the benefits of limiting supply.



Another detailed report \cite{castiglione2016tncs} by San Francisco Transportation Authority  provides information on the size, location, and time-of-day characteristics of TNC activities in San Francisco. The follow-up report  \cite{castiglione2018tncs} identifies the impact of TNC activities on roadway congestion in San Francisco County. It shows that after subtracting the impact of employment growth, population change, and network capacity change, TNCs accounted for  51 percent of the increase in vehicle hours of delay, 47 percent of increase in VMT, and 55 percent of the average speed decline  between 2010 and 2016.  Moreover, ``TNC trips are concentrated in the densest and most congested parts of San Francisco including the downtown and northeastern core of the city. At peak periods, TNCs are estimated to comprise 25 percent of vehicle trips in South of Market.'' The report cites studies showing that ``between 43 percent and 61 percent of TNC trips substitute for transit, walk, or bike travel or would not have been made at all.'' 


This paper evaluates two policies regulating TNCs: a minimum driver wage, and a cap on the  number of drivers or vehicles. We analyze the  impacts of these policies on several aspects of the the app-based 
ride-hailing market, including  ride prices and driver wages established by the platform,  the incentives of passengers and drivers, vehicle occupancy rate, and platform rent or profit. We use a model to  determine 
the arrival of passengers, number of drivers, ride prices and platform commissions, conditioned on the exogenous regulatory policy.  The model employs 
 a queuing theoretic model with dynamic matching of passengers and drivers,  an equilibrium model  that predicts the long-term average arrivals of passengers and drivers, and an optimization model that captures  platform decision-making. We summarize the key results.
\begin{itemize}
\item Imposing a minimum wage will motivate TNCs to hire {\em more} drivers, and passengers to enjoy {\em faster} and {\em cheaper} rides, while TNC rent or profit shrinks. In contrast with the traditional economic model \cite{Neumark},  raising the minimum wage   will benefit both  drivers and passengers, while TNC rents will decline. This counter-intuitive result holds for a large regime of model parameters, and it occurs because the quality of service  increases with the number of drivers. Consequently, by hiring more drivers the platform  improves the quality of service (pickup time) and attracts more passengers. For certain values of the minimum wage, the increased sales volume   outweighs the increased labor cost.  
\item Contrary to  common belief,   a cap on the number of drivers will  hurt  driver earnings.   This is because when fewer drivers are permitted, the platform will hire cheaper labor by reducing  driver pay. In other words, the benefit of limiting the driver supply is retained by the platform.    
\end{itemize}

Aside from these results, we also present variants of our model to analyze platform subsidy, platform competition and autonomous vehicles.

*************************
{\bf Related Works}: There are many studies of ride-hailing platforms. A major consideration is to evaluate decisions that maximize platform profit. Using 
a queuing theoretic model is proposed in \cite{banerjee2015pricing} to study the optimal pricing of ride-hailing platforms. It shows that the throughput and profit under dynamic pricing strategy can not exceed that under the optimal static pricing strategy that is agnostic to stochastic dynamics of demands. On the other hand, it also shows that dynamic pricing is much more robust to fluctuations in systems parameters compared to static pricing. Therefore, the platform can use dynamic pricing to realize the benefits of optimal static pricing without perfect knowledge of system parameters. A similar problem is studied by \cite{cachon2017role}, with a focus focus on the self-scheduling capacity of for-hire drivers. It shows the additional flexibility of drivers is beneficial to both  platforms, consumers and drivers.  It also suggests that when some periods have predictably higher demand than others (e.g., a rainy evening),  static pricing is hard to find service at peak demand times, so that surge pricing is likely to benefit all stakeholders in this case.  In the same vein, Bai (2017) \cite{bai2018coordinating}  suggests dynamic pricing for  the platform to maximize the profit across different time periods when the underlying operating characteristics can change significantly.   Taylor (2018)  shows in \cite{taylor2018demand} that platform pricing can be more complicated when there is uncertainty in passenger's valuation or driver's opportunity cost. 
Ban developed a general economic equilibrium model to evaluate the impacts of ride-hailing services on the  deadhead miles and traffic congestion \cite{ban2018gan}. 
In addition, ride-hailing platforms are also closely inspected in the economic literature as a special case of two-sided platform. See \cite{rysman2009economics} and \cite{rochet2006two} for a  summary of literature in two sided-platforms, and \cite{weyl2010price} for a general theory of monopoly pricing in multi-sided platforms. 





The literature on regulatory policies of app-based ride-hailing marketplace is relatively limited. Gurvich (2016) \cite{gurvich2016operations} considered a ride-hailing platform that manages a group self-scheduling drivers to serve the time-varying demand. It shows that under a wage floor, the platform starts to limit the agent flexibility by restricting the number of agents that can work in some time intervals. Optimal pricing under exogenous wage is considered in \cite{hu2017price}. It shows that when the platform sets the trip price under an exogenously  given wage, the optimal price has a U-shape relation with respect to wage: as driver wage increases, the ride price first decreases, and then increases. However, the key limitation of this result is that it assume that the platform always sets driver pays at an exogenous wage, even if this wage is below the profit maximizing level. In practice, the platform optimizes {\em both} price and wage under a wage floor, and the first half of the U-shape never appears based on the model of \cite{hu2017price} (see more discussions in Section \ref{maintheoremsec}). 



The closest work to ours is reported in Parrott and Reich \cite{parrott2018earning}. The authors use the administrative data of TNCs collected by the New York City Taxi and Limousine Commission (TLC) to examine the likely impact of the TCL's proposed regulatory policies \cite{nycdoc}. By numerical simulation, they show that the proposed policy will increase driver earnings by 22.5 percent, while the passengers will only experience moderate increase of trip fare (less than 5 percent ) and waiting times (12 to 15 seconds). However, our analysis shows that both the trip cost  and the waiting time will decrease. This is because in our model we assume that the passengers are sensitive to the pickup time of the ride-hailing services, which is not captured in \cite{parrott2018earning}.


*****************
 
